Breaking Through the Full-Duplex Wi-Fi Capacity Gain

In this work we identify a seminal design guideline that prevents current Full-Duplex (FD) MAC protocols to scale the FD capacity gain (i.e. 2x the half-duplex throughput) in single-cell Wi-Fi networks. Under such guideline (referred to as 1:1), a MAC protocol attempts to initiate up to two simultaneous transmissions in the FD bandwidth. Since in single-cell Wi-Fi networks MAC performance is bounded by the PHY layer capacity, this implies gains strictly less than 2x over half-duplex at the MAC layer. To face this limitation, we argue for the 1:N design guideline. Under 1:N, FD MAC protocols 'see' the FD bandwidth through N>1 orthogonal narrow-channel PHY layers. Based on theoretical results and software defined radio experiments, we show the 1:N design can leverage the Wi-Fi capacity gain more than 2x at and below the MAC layer. This translates the denser modulation scheme incurred by channel narrowing and the increase in the spatial reuse offer enabled by channel orthogonality. With these results, we believe our design guideline can inspire a new generation of Wi-Fi MAC protocols that fully embody and scale the FD capacity gain.

==> fdchannel.tex <==
\tikzstyle{RectObject}=[rectangle,fill=white,draw,line width=0.5mm]
\begin{figure}
\begin{tikzpicture}[scale=0.775,transform shape]
%=========================> Drawing the channels
  \draw (0,-1) node[left] {ST}  -- (7.5,-1) ;
  \draw (0,0) node[left] {PT} --  (7.5,0)  ;
  \draw[-latex, line width=0.35mm] (0,-2) -- (9.5,-2) node[below]{Time};
%=========================> Drawing PRIMARY transmission
%------------------------------------------------> First frame
  %--------> headers 1.1 (width = 0.7)
  \draw[line width=0.3mm] (0.4, 0) rectangle (1.1, 0.5) node[midway] {$H$} ;

  %--------> payload 1.1 (width = 3.7)
  \draw [<->] (1.1, 0.8) -- (4.8, 0.8) node[midway, above] {$T_P$};
  \draw[line width=0.3mm,fill=black!15] (1.1, 0) rectangle (4.8, 0.5) node[midway] {$P$ (Bytes)} ;

  %--------> sifs 1.1 (width = .8)
  \draw[line width=0.3mm] (4.8, 0) -- (5.6, 0) node[anchor=center, midway,above] {\scriptsize{$SIFS$}} ;

  %--------> ack 1.1 (width = 1.4)
  \draw[line width=0.3mm] (5.6, 0) rectangle (7, 0.5) node[midway] {$T_{ACK}$};

  %--------> difs 1.1 (width = 1.5)
  \draw[line width=0.3mm] (7, 0) -- (8.5, 0) node[anchor=center, midway,above] {$DIFS$};
%==================================================> Drawing secondary transmission events
%------------------------------------------------> First frame
  %--------> headers 2.1 (width = .7)
  \draw[line width=0.3mm] (1.3, -1) rectangle (2, -0.5) node[midway] {$H$} ;
  %--------> payload 2.1 (width = 3.7)
  \draw[line width=0.3mm, fill=black!15] (1.9, -1) rectangle (4.8, -0.5) node[midway] {$P'$ (Bytes)} ;
  % NOTE THAT HERE WE JUST COPY ABOVE FRAME AND MULTIPLY OR REPLACE Y AXIS BY -1
  %--------> sifs 1.1 (width = .8)
  \draw[line width=0.3mm] (4.8, -1) -- (5.6, -1) node[anchor=center, midway,above] {\scriptsize{$SIFS$}} ;

  %--------> ack 1.1 (width = 1.4)
  \draw[line width=0.3mm] (5.6, -1) rectangle (7, -0.5) node[midway] {$T_{ACK}$};

  %--------> difs 1.1 (width = 1.5)
  \draw[line width=0.3mm] (7, -1) -- (8.5, -1) node[anchor=center, midway,above] {$DIFS$};

%=====================================================> CREATING TIME SLOTS
%  \draw[dotted] (0,0) --  (0, -2) node[below]{$t_0$};
  \draw[dotted] (0.4,0) --  (0.4, -2) node[below]{$t_0$};
  \draw[dotted] (1.1,0) --  (1.1, -2) node[below]{$t_1$};
  \draw[dotted] (1.3,0) --  (1.3, -2) node[below]{$t_2$};
  \draw[dotted] (1.9, 0) --    (1.9, -2) node[below]{$t_3$};
  \draw[dotted] (8.5,0) --  (8.5, -2) node[below]{$t_4$};
\end{tikzpicture}
\caption{The \emph{expected} payload a PbP-EDCA secondary channel ($c=1$)
  added at each time slot of the primary channel ($c=0$): 
  $E[L_{\sigma}]$, $E[L_{suc}]$, and $E[L_{col}]$ bytes for time slots of
  the types ``idle'' ($t_4$ to $t_5$), ``successful'' ($t_5$ to $t_6$) and
  ``collision'' ($t_6$ to $t_7$), respectively. Transmissions started at
  $t_1$ and $t_5$ wait one and three 802.11 slots, respectively.  \footnotesize{\copyright Saulo J. B. de Queiroz}.}
\label{fig:pbpcapacity}
\end{figure}

